Estimating Causal Effects with Hidden Confounding using Instrumental Variables and Environments

Recent works have proposed regression models which are invariant across data collection environments. These estimators often have a causal interpretation under conditions on the environments and type of invariance imposed. One recent example, the Causal Dantzig (CD), is consistent under hidden confounding and represents an alternative to classical instrumental variable estimators such as Two Stage Least Squares (TSLS). In this work we derive the CD as a generalized method of moments (GMM) estimator. The GMM representation leads to several practical results, including 1) creation of the Generalized Causal Dantzig (GCD) estimator which can be applied to problems with continuous environments where the CD cannot be fit 2) a Hybrid (GCD-TSLS combination) estimator which has properties superior to GCD or TSLS alone 3) straightforward asymptotic results for all methods using GMM theory. We compare the CD, GCD, TSLS, and Hybrid estimators in simulations and an application to a Flow Cytometry data set. The newly proposed GCD and Hybrid estimators have superior performance to existing methods in many settings.

==> figs/exp2-res.tex <==
\begin{table}

\caption{Estimation result for AKT $\to$ ERK.}
\centering
\begin{tabular}{|c|c|c|c|}
\hline
\multicolumn{1}{|l|}{} & GCD(CD) & IV                & OLS               \\ \hline
Coefficient            & 0.57    & 1.11              & 0.96              \\ \hline
P value                & 0.07    & \textless{}0.0001 & \textless{}0.0001 \\ \hline
\end{tabular}
\end{table}




==> figs/exp3-res.tex <==
\begin{table}

\caption{Estimation result for PIP2 $\to$ Plcg.}
\centering
\begin{tabular}{|c|c|c|c|}
\hline
\multicolumn{1}{|l|}{} & GCD(CD) & IV                & OLS               \\ \hline
Coefficient            & 1.88    & 0.42              & 0.31              \\ \hline
P value                & 1       & \textless{}0.0001 & \textless{}0.0001 \\ \hline
\end{tabular}
\end{table}




==> figs/tab-res.tex <==
\begin{table}

\caption{Causal relations found by GCD and CD}
\centering
\begin{tabular}{|c|c|c|}
\hline
Response & Causality found by GCD       & Causality found by CD \\ \hline
Akt      & Mek, Erk, PKA                & Erk, PKA              \\ \hline
Erk      & Mek, Akt, PKA, PKC, P38, Jnk & Raf, Akt, P38         \\ \hline
Jnk      & P38                          & P38, PKC              \\ \hline
Mek      & Raf                          & Raf                   \\ \hline
P38      & Mek, PIP3, PKC, Jnk          & PKC, Jnk              \\ \hline
PIP2     & PIP3                         & PIP3                  \\ \hline
PIP3     & PIP2                         & -                     \\ \hline
PKA      & PIP3, Akt                    & Akt                   \\ \hline
PKC      & PLCg, PIP3, Erk, Akt, P38    & P38                   \\ \hline
PLCg     & PIP2, PKA, Jnk               & -                     \\ \hline
Raf      & Mek, Akt                     & Mek, Akt              \\ \hline
\end{tabular}
\end{table}

==> figs/tab_mean_var.tex <==
\begin{table}

\caption{Mean and variance change for candidate input variables after the interventions. The changes were measured in portion.}
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
\multicolumn{1}{|l|}{}     & AKT   & PKC   & PIP2  & MEK   \\ \hline
Mean change in portion     & +0.05 & +0.72 & -0.64 & +0.67 \\ \hline
Variance change in portion & +0.20 & +0.41 & -0.15 & +2.53 \\ \hline
\end{tabular}
\end{table}




==> figs/tab_mek_raf.tex <==
\begin{table}

\caption{Mean and variance changes for Mek and Raf}
\centering
\begin{tabular}{|c|c|c|c|}
\hline
\multicolumn{1}{|l|}{} & GCD(CD)           & IV                & OLS               \\ \hline
Coefficient            & 0.94              & 0.60              & 0.31              \\ \hline
P value                & \textless{}0.0001 & \textless{}0.0001 & \textless{}0.0001 \\ \hline
\end{tabular}
\end{table}



